Singularity-aware motion planning for multi-axis additive manufacturing

Multi-axis additive manufacturing enables high flexibility of material deposition along dynamically varied directions. The Cartesian motion platforms of these machines include three parallel axes and two rotational axes. Singularity on rotational axes is a critical issue to be tackled in motion planning for ensuring high quality of manufacturing results. The highly nonlinear mapping in the singular region can convert a smooth toolpath with uniformly sampled waypoints defined in the model coordinate system into a highly discontinuous motion in the machine coordinate system, which leads to over-extrusion / under-extrusion of materials in filament-based additive manufacturing. The problem is challenging as both the maximal and the minimal speeds at the tip of a printer head must be controlled in motion. Moreover, collision may occur when sampling-based collision avoidance is employed. In this paper, we present a motion planning method to support the manufacturing realization of designed toolpaths for multi-axis additive manufacturing. Problems of singularity and collision are considered in an integrated manner to improve the motion therefore the quality of fabrication.

==> tex/intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{secIntro}

\textit{Additive manufacturing} (AM) has a profound impact on a large amount of fields to build fast prototypes and fabricate products with complex geometry shape~\cite{GIBSON_BOOK14}. The normal setup of 3D printing contains three axis which accumulates material layer-by-layer along vertical direction of sliced planes. This kind of configure, so-called 2.5D printing, is relatively low cost and easy to apply. However, the limited \textit{degree-of-freedoms} (DOFs) in motion restricts the nozzle to move freely in 3D space. This naturally brings the problem of heavy supporting structures requirement for overhang region and staircase artifacts 
at the high-curvature surface.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/pipeline.jpg}
    \caption{Pipeline of MAAM system, which includes three parts: (a) curved-layer slicing and tool-path planning, (b) post-processing G-code generator to ensure collision-free axis motion and dynamic nozzle control, (c) hardware which enable 3D space nozzle motion and final manufacturing process. We focus on the second step.}
    \label{fig:pipeline}
\end{figure}

Recent years, 3D printing systems including multi-axis motion have been developed to overcome the drawbacks of flat layer-based printing~\cite{Dai_ACM18,XIE_RCIM20}. These multi-DOF system can re-orientate the platform and nozzle to make material deposition direction align with the normal of curved surface. Thus, they enable advanced functionality such as support-free printing, enhancement in strength, etc. On the other hand, this technology increases complexity of both software and hardware. Different from planar-layer based method, the \textit{multi-axis additive manufacturing} (MAAM) system not only requires advanced algorithm to cut model into curved working surface and toolpath, but also the high DOFs bring the challenge into the motion control. 

In our previous research~\cite{FANG_SIGG20}, two kinds of multi-axis printing hardware and advanced curve-layer slicing algorithm were developed, while this paper focuses on the proper control for axis motion. The post-processing step (shows in Fig.~\ref{fig:pipeline}) is important to make sure the successful printing and the quality of printed objects. There are 3 main properties of MAAM different from planar-based AM: 

1) \textbf{Curved slicing and toolpath.} Aligning material along 3D tool-path needs to avoid collision between nozzle, printed part and platform.
   
2) \textbf{Multi-axis motion control.} Accumulating materials smoothly and continuously in the \textit{workpiece coordinate system} (WCS) to ensure the quality and strength of models.

3) \textbf{Non-uniform layer thickness.} The layer height varies continuously, which requires a dynamic control in nozzle extrusion to generate proper material volume for each waypoint.

Focusing on the 2nd part, we develop a general post-processing method for multi-axis 3D printing system to generate specialized G-code which controls the machine to have a collision-free and smooth motion to complete the printing task. In particular, the technical contribution of this paper are as follows:

\begin{itemize}
    \item A general post-processing method in MAAM process. Specialized G-code is generated by considering the multi-axis motion and synchronized nozzle extrusion.
    \item A searching-based shortest-path planning algorithm for adjusting nozzle orientation to generate a smooth and collision-free motion. 
    \item Singularity in coordinate mapping of high-DOFs system is optimized to forbid enormous change in axis motion, and we solve the coupling problem of collision elimination and singularity optimization. 
    \item We build a nozzle control theory considering the filament volume and hysteresis property.
\end{itemize}

The rest of this work is organized as follows. Sec.\ref{secRelatedWork} presents the related work on multi-axis additive manufacturing system and trajectory planning for high DOFs motion. In Sec.\ref{secProblemDefinition}, kinematics for multi-axis machine and the problem statement in motion planning are discussed. In Sec.\ref{secMotionPlanning}, we then give the solution for collision-free and smooth motion planning. Sec.\ref{secResultComparation} presents the validation and experiment result. Our paper ends with the summary and discussion in Sec.\ref{secConclusion}.


==> tex/relatedWork.tex <==
\section{Related work}\label{secRelatedWork}

The most popular setups of traditional FDM printers are Cartesian and Delta. Their common feature is that the printing head moves linearly in the X, Y, and Z direction. Planar printing usually requires support structures as the deposition is made in one direction from bottom to top. At the same time, the weak linkage between layers limits the strength of printing parts, and the staircase effect decreases the surface quality. A lot of researchers attempt to solve the above problems by introducing more freedom into the manufacturing cells. 

Luo et al.\cite{LUO_IEEE20} added extra movement axes and achieved multi-orientation printing to enhance the strength of the printed parts, while only simple models are fabricated in their experiments and no detail about the printing process. Xu et al.\cite{XU_CAD19} conducted layer decomposition and contour-parallel path generation by calculating geodesic distance field on the mesh. The verification is base on a prototype multi-axis FDM system, however, there is less detail about fabrication issues. Dai et al.\cite{Dai_ACM18} proposed a pipeline of conducting support-free printing with a robotic arm. However, some artifacts occur as relatively low positioning accuracy. The 5AxisMaker is a popular desktop 5-axis 3D fabrication system on the market. Two students from the Zurich University of Applied Sciences, Oliver Tolar and Denis Herrmann developed a 6-axis 3D printer for eliminating support structures entirely. 

There is a large amount of research on conventional multi-axis CNC manufacturing technology. The main consideration contains collision and singularity issues. Jung et al.\cite{JUNG_02JMPT} used the tool retracts to avoid the points near the singular configuration. This modification introduce interrupts in the cutting path, which is therefore undesirable in simultaneous 5-axis machining. A. Affouard  et al.\cite{AFFOUARD_IJMTM04} adopted the concept of the singular cone and deformed the tool-path to avoid this cone. Sorby \cite{SORBY_07IJMTM} displayed a clear definition of and provided two types of solution for singularity issues which are similar with our related methods for multi-axis 3D printing machine. Chu et al.\cite{CHU_IJPR16} proposed an analytical scheme for identifying singular configuration and developed an algorithm to compute the cutter path across the neighborhood of the singular points such that the computed path tracks the desired tool path within a controllable error. This, however, method stems from control theory and is based on real-time feedback of joint angle. And it is not suitable for machines whose post-processor and NC (Numerical control unit) is separated. 

Mahadevan et al.\cite{Mahadevan_CAD03} presented a algorithm to generate collision-free 5-axis CNC toolpath based on the visibility data from graphics hardware and the manufacturing limitation was considered. Wang et al.\cite{WANG_CAD07} presented an approach that automatically generates a interference-free toolpath and it guarantees the angular-velocity compliance by computing and manipulating visibility maps. Xu et al.\cite{XU_IJMS19} proposed a kinematics performance-oriented smoothing method to plan the tool orientations and the collision-free also be ensured. Lacharnay et al.\cite{LACHARNAY_CAD15} used the potential field to push the tool away from the obstacle when the tool is close to the obstacle, which reduces requirements of computing the collision-free tool-path. Mirzendehdel et al.\cite{MIRZENDEHDEL_CAD20} adopted the topology optimization to eliminate the inaccessibility of manufacturing.

However, the shape of the 5-axis CNC cutter is a slim cylinder, while the printing head of multi-axis 3DP is always huge, including heat block, fan, and temperature sensor. As a result, the accessibility space of multi-axis 3DP is more narrow than the counterpart of CNC. Meanwhile, the subtractive manufacturing is conducted on a solid blank with surface-cutting performance, but the additive fabrication accumulates each material volume on a platform step by step. So collision checking of 3DP is more complex and time-consuming. What's more, although there are lots of research on singularity and collision issues, rare work focuses on the coupling problem of singularity and collision. And the extrusion value of each waypoint needs to be controlled carefully, while the CNC machining does not need to consider this issue as the isotropic property of the material. Our work focuses on the supporting pipeline of the multi-axis 3DP system from the numerical information to the final printing parts.
